Fortran MPI Checkerboard Code for SU(3) Lattice Gauge Theory I

We document Fortran MPI checkerboard code for Markov Chain Monte Carlo simulations of pure SU(3) lattice gauge theory with the Wilson action on a D-dimensional double-layered torus. This includes the usual torus with periodic boundary conditions as an optional case. We use Cabibbo-Marinari heatbath checkerboard updating. Parallelization on sublattices is implemented in all D directions and can be restricted to less than D directions. The parallelization techniques of this paper can be used for any model with interactions of link variables defined on plaquettes.

==> Tables1/table01old.tex <==
\begin{table}[th] % Collect in SU3V1DLT folders.
\centering
\caption{\label{tab01}{Runs with ${\tt mpifactor}= 2$ at $\beta=5.7$ 
with identical random numbers on $4^4$ sublattices. Collect in SU3V1DLT 
folders. The $\tt msmpi=1$ comparison run in SU3VPBC (should be 
converted to checkerboard). \hfil
First part: 1-hit Cabibbo-Marinari. \hfil
Second part: Full Cabibbo-Marinari (problematic for parallelization).
\hfil\break
The lower part does the same comparison with MPI data from code with 
usual periodic boundary conditions kept in SU3VPBC and the $\tt msmpi
=1$ comparison run from STMCnew.}} \medskip
\begin{tabular}{|c|c|c|c|c|}
\hline
{\tt msmpi}&{\tt ndmpi}& CPU time  & {\tt actm}    & $Q$  \\ \hline
    1      &   $-$     &     35 m  & 0.53755 (23) & $-$  \\ \hline
    2      &    1      &     45 m  & 0.53802 (20) & 0.12 \\ \hline
{\tt msmpi}&{\tt ndmpi}& CPU time  & {\tt actm}    & $Q$  \\ \hline
    1      &   $-$     &     35 m  & 0.53755 (23) & $-$  \\ \hline
    2      &    1      &     45 m  & 0.53767 (20) & 0.69 \\ \hline
    4      &    2      &     99 m  & 0.53767 (20) & 1.00 \\ \hline
{\tt msmpi}&{\tt ndmpi}& CPU time  & {\tt actm}    & $Q$  \\ \hline
    1      &   $-$     &     35 m  & 0.53772 (16) & $-$  \\ \hline
    2      &    1      &     45 m  & 0.53772 (17) & 0.99 \\ \hline
    4      &    2      &     99 m  & 0.53772 (17) & 1.00 \\ \hline
\end{tabular}
\end{table}


==> Tables1/table03a.tex <==
\begin{table}[th] % Collect in SU3V2DLT folders.
\centering
\caption{\label{tab05}{Runs with n MPI processes, ${\tt mpifactor}=$nf, 
{\tt ndmpi}=nd on a double-layered $8^3\,4$ lattice at $\beta=5.55$.
As table03, but on unxc02 with ordered starts. }} 
\medskip
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
np &nf &nd &{\tt nl1}&{\tt nl2}&{\tt nl3}&{\tt nl4}
                       &  {\tt actm}   & $Q$  \\ \hline
 2 & 1 & 1 & 8& 8& 8& 4& 0.510676 (31) & $-$  \\ \hline
 4 & 2 & 1 & 4& 8& 8& 4& 0.510665 (37) & 0.?? \\ \hline
 8 & 2 & 2 & 4& 4& 8& 4& 0.510646 (38) & 0.?? \\ \hline
16 & 2 & 3 & 4& 4& 4& 4& 0.510605 (33) & 0.?? \\ \hline
\end{tabular}
\end{table}


==> Tables1/table03b.tex <==
\begin{table}[th] % Collect in SU3V2DLT folders.
\centering
\caption{\label{tab05}{As table03
Runs with np MPI processes, ${\tt mpifactor}=$nf, {\tt ndmpi}=nd on a 
double-layered $8^3\,4$ lattice at $\beta=5.55$, disordered starts.
As table03, but runs on unxc02. }} 
\medskip
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
np &nf &nd &{\tt nl1}&{\tt nl2}&{\tt nl3}&{\tt nl4}
                       &  {\tt actm}   & $Q$  \\ \hline
 2 & 1 & 1 & 8& 8& 8& 4& 0.510596 (34) & $-$  \\ \hline
 4 & 2 & 1 & 4& 8& 8& 4& 0.510634 (30) & 0.?? \\ \hline
 8 & 2 & 2 & 4& 4& 8& 4& 0.510665 (36) & 0.?? \\ \hline
16 & 2 & 3 & 4& 4& 4& 4& 0.510585 (26) & 0.?? \\ \hline
\end{tabular}
\end{table}


==> Tables1/table04.tex <==
\begin{table}[th] % Collect in old SU3V1DLT folder.
\centering
\caption{\label{tab04}{Polyakov absolute values for some of 
the runs of the previous table. Collect in SU3V1DLT folders.}} 
\medskip
\begin{tabular}{|c|c|c|c|}
\hline
$\beta$&{\tt msmpi}& $|P|$  &$Q$ \\ 
\hline
  5.65 &  1   &0.01584 (32)& $-$ \\ 
  5.65 &  2-l &0.01580 (14)&0.91 \\ 
\hline
\end{tabular}
\end{table}

